Bit-Line Computing for CNN Accelerators Co-Design in Edge AI Inference

By supporting the access of multiple memory words at the same time, Bit-line Computing (BC) architectures allow the parallel execution of bit-wise operations in-memory. At the array periphery, arithmetic operations are then derived with little additional overhead. Such a paradigm opens novel opportunities for Artificial Intelligence (AI) at the edge, thanks to the massive parallelism inherent in memory arrays and the extreme energy efficiency of computing in-situ, hence avoiding data transfers. Previous works have shown that BC brings disruptive efficiency gains when targeting AI workloads, a key metric in the context of emerging edge AI scenarios. This manuscript builds on these findings by proposing an end-to-end framework that leverages BC-specific optimizations to enable high parallelism and aggressive compression of AI models. Our approach is supported by a novel hardware module performing real-time decoding, as well as new algorithms to enable BC-friendly model compression. Our hardware/software approach results in a 91% energy savings (for a 1% accuracy degradation constraint) regarding state-of-the-art BC computing approaches.

==> tableCompression.tex <==
\begin{table}
\centering
\caption{Compression rate using Huffman Enconding.}
\begin{tabular}{c|c|c|c|c|c}
Bits         & \textbf{AlexNet} & \textbf{MobileNet} & \textbf{LeNet} & \textbf{VGG16} & \textbf{Xception} \\ \hline
\textbf{4} & -                & 2.86               & -              & 3.81           & 3.62              \\ \hline
\textbf{5} & -                & 2.44               & -              & 1.87           & 2.83              \\ \hline
\textbf{6} & 2.90             & 2.50               & 1.57           & 0.99           & 2.46              \\ \hline
\textbf{7} & 2.38             & -                  & 0.85           & -              & -                 \\ \hline
\textbf{8} & 0.80             & -                  & -              & -              & -                
\end{tabular}
\label{tab:compr}
\end{table}

==> table_wordlevelparallelism.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Multiplexers M1 and M2 output for the two word modes: 1 word of 16 bits or 2 words of 8 bits.}
\begin{tabular}{l|c|cc}
\multicolumn{1}{c|}{Word mode}          & byte                             & M1                           & M2                          \\ \hline
\multirow{2}{*}{16 bits - 1 word}  & bit\textless{}15:8\textgreater{} & S\textless{}15\textgreater{} & C\textless{}7\textgreater{} \\
                                   & bit\textless{}7:0\textgreater{}  & S\textless{}8\textgreater{}  & CIN                         \\ \hline
\multirow{2}{*}{8 bits  - 2 words} & bit\textless{}15:8\textgreater{} & S\textless{}15\textgreater{} & CIN                         \\
                                   & bit\textless{}7:0\textgreater{}  & S\textless{}7\textgreater{}  & CIN                        
\end{tabular}
\label{tab:wl}
\end{table}
